Towards Robust, Locally Linear Deep Networks

Deep networks realize complex mappings that are often understood by their locally linear behavior at or around points of interest. For example, we use the derivative of the mapping with respect to its inputs for sensitivity analysis, or to explain (obtain coordinate relevance for) a prediction. One key challenge is that such derivatives are themselves inherently unstable. In this paper, we propose a new learning problem to encourage deep networks to have stable derivatives over larger regions. While the problem is challenging in general, we focus on networks with piecewise linear activation functions. Our algorithm consists of an inference step that identifies a region around a point where linear approximation is provably stable, and an optimization step to expand such regions. We propose a novel relaxation to scale the algorithm to realistic models. We illustrate our method with residual and recurrent networks on image and sequence datasets.

==> src/intro-2.tex <==
\section{Introduction}

%\ghl{Focus on linearities, instead of intimidating ``Jacobian''. Change the least favorable prior to mini-max methods like Tatsu's paper.}

The derivative of a predictor function with respect to its inputs is an object of utmost importance in machine learning. Although less prominent in the literature that derivatives with respect to parameters, those with respect to inputs are a crucial manifestation of the behavior of a function, since it defines sensitivity of a function with respect to the inputs. 
For example, it is frequently used to derive explanations for model predictions~\citep{baehrens2010explain, simonyan2013deep, sundararajan2017axiomatic, smilkov2017smoothgrad}; 
as motivated by Taylor expansion, first-order approximation with derivatives is a ubiquitous choice of local approximation~\citep{rifai2012generative, goodfellow14, wang2016learning, koh2017understanding, alvarez2018towards}.
Besides, the derivatives are also exploited to characterize learning objectives~\citep{gulrajani2017improved, bellemare2017cramer, mroueh2017sobolev}, which typically compose penalties according to a functional class defined by the derivatives. 
Note that the `derivatives' discussed in this paper are about the output of a neural network with respect to the input rather than its parameters. 

%and conduct Bayesian inference~\cite{liu2016stein}
%is also used to compose penalty with respect to some functional classes, typically when the functional classes are (re-)defined on the Jacobian\cite{liu2016stein}.
%\dam{Again, cite needed}


However, the derivatives of functions parameterized by deep learning models are in general not stable~\citep{ghorbani2017interpretation}. The state-of-the-art deep learning models~\citep{he2016deep, huang2017densely} typically \update{over-parametrize a function to fit the data~\citep{zhang2016understanding}, which might yield an unstable function as a side effect. 
Such instability is reflected on both the function values~\citep{goodfellow14} and the derivatives~\citep{ghorbani2017interpretation, alvarez2018robustness}.}
As a direct result of unstable derivatives, methods in deep learning building upon first-order approximations inherently lack robustness~\citep{ghorbani2017interpretation, alvarez2018robustness}.

While conceptually similar, the phenomenon of unstable derivatives is different from adversarial examples that flip predictions~\citep{goodfellow14} since they describe two orthogonal aspects of instability: the sensitivity of a function versus the value of a function. 
Indeed, taking $1$-dimensional functions for example, a line yields constant derivatives but unstable outputs if the derivative is large, and a sinusoidal function with high frequency has bounded output but unstable derivatives. 
%\ghl{remove the following?} Methodologically, the state-of-the-art adversarial learning approach~\citep{madry2017towards} even relies on the Jacobian of deep networks for both attacking and defending adversarial examples, while we are not aware of any prior work to ``protect'' the Jacobian.

%\dam{in what sense? solved?}
%\dam{minimax principle has a specific meaning (interchangeabilty of min and max), which I dont think is what you mean here}

While robust estimation is \update{mostly formulated as a minimax problem, which minimizes a ``maximizing adversary'' within a set of choices, such framework is in general intractable for learning stable derivatives in modern neural networks.
Such minimax problem has been studied} in the context of classic robust regression~\citep{xu2009robust}, distributionally robust optimization~\citep{namkoong2017variance, hashimoto2018fairness} and adversarial learning~\citep{madry2017towards}.
If applying the minimax principle for robust derivatives, the inner-maximization problem for the ``maximally distorted derivatives'' is itself a challenging optimization problem, where even a gradient-based method is not applicable since it requires the Hessian of deep networks.

Instead, here we focus on neural networks with piecewise linear activations to make the problem tractable. 
The special structure of this class of networks allows us to derive explicit characterizations of their functional properties, and develop inference algorithms to identify lower bounds on the $\ell_p$ \emph{margin} --- the maximum radius of $\ell_p$-norm balls around a point where derivatives are provably stable.
We further investigate the special case $p=2$, in which the lower bound has an analytical solution, allowing us to formulate a regularization problem to maximize it.
Since the induced objective is inherently rigid and non-smooth, we further relax the learning problem with a novel derivation similar to the primal of support vector machines (SVM)~\citep{vapnik1995estimation, cortes1995support}.

Both the inference and learning algorithms require computing the gradient of each neuron with respect to the input, which poses a significant computational challenge. 
By utilizing piecewise linearity of the networks, given $D$-dimensional data, we propose a novel perturbation algorithm that collects all the \emph{exact} gradients with only forwarding $O(D)$ carefully crafted samples \emph{in parallel} --- without any call to back-propagation. 
When the GPU memory cannot fit $O(D)$ samples in one batch, we develop an unbiased approximation to the objective with a random subset of such samples.

Empirically, we examine our inference and learning algorithms with fully-connected (FC), residual (ResNet)~\citep{he2016deep}, and recurrent (RNN) networks on image and time-series datasets with quantitative and qualitative experiments. 
The main contributions of this work are as follows:
\vspace{-2mm}
\begin{itemize}
\item Inference algorithms that identify input regions of neural networks, with piecewise linear activation functions, that are provably stable.
\vspace{-1mm}
\item A novel learning criterion that effectively expand regions of provably stable derivatives.
\vspace{-1mm}
\item Novel perturbation algorithms that scale computation to high dimension data.
\vspace{-1mm}
\item Rich empirical study on the applicability of the methods with various types of networks.
\vspace{-2mm}
\end{itemize}

%\dam{The intro is missing a stronger last parapraph, a "punchline". Either explcitily listing contributions or emphasizing nivelyy of the approach, etc.}

%\ghl{The implementation is in Supplementary Material}

% up to here
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\iffalse
Fortunately, due to special functional structure of neural networks with piece-wise linear activation, we discover algorithms that can identify regions where the Jacobian is stable. 
Specifically, by exploiting the convexity of a locally linear region, we are able to create a binary search algorithm that find certificate on maximum directional perturbation and $\ell_1$ ball around a point $\bx$ that Jacobian is guaranteed to be stable. 
In addition, by further exploiting the geometry of locally linear regions, we develop novel analytical algorithm to find the exact certificate on the maximum $\ell_2$ ball around $\bx$ where Jacobian is stable; the algorithm requires computation of the Jacobian of all the neurons with respect to input, which yields a giant computational challenge: naively calling back-propagation for each neuron is intractable. In contrast, we create a novel algorithm that computes the exact Jacobian of all the neurons with respect an input axis by feeding 2 carefully crafted perturbations to the network (in parallel), which does not even require a single call to back-propagation. The computational algorithm can be amortized and parallelized among the input axes that the complexity given $D$ dimensional data is $D+1$ calls to forward pass in parallel.

With the capability to certify the size of locally linear regions, we further develop learning algorithms to expand such locally linear region. Due to the difficulty of the optimization problem, we develop a novel relaxation based on the derivation of primal support vector machine (SVM)~\cite{vapnik1995estimation, cortes1995support}, where the final formulation is resemble to transductive/semi-supervised SVM (TSVM)~\cite{vapnik1977tsvm, bennett1999semi}. The learning algorithm has the same complexity as the $\ell_2$ certificate problem, which can be computationally challenging in a training scenario when the $D+1$ forward pass cannot be parallelized in one batch (e.g., deep   model on large image). As a result, we develop an unbiased approximate learning algorithm that scales to such high dimensional setting.  
\fi

==> src/intro.tex <==
\section{Introduction}


Given a function $f$ mapping from $\mathbb{R}^D$ to $\mathbb{R}^L$ The Jacobian of a function $J_\bx f(\bx) \in \mathbb{R}^{L\times D}$\footnote{Jacobian is a matrix where each row corresponds to the gradient of each output axis.} (i.e., gradient when output is multivariate) is one of the most important statistics in machine learning, which is used for first-order function approximation~\cite{rifai2012generative, koh2017understanding, alvarez2018towards}, to train GANs~\cite{goodfellow2014generative, dumoulin2016adversarially, arjovsky2017wasserstein, isola2017image}, and to derive explanations for model prediction~\cite{baehrens2010explain, simonyan2013deep, sundararajan2017axiomatic, smilkov2017smoothgrad}. However, such statistics is in general not stable in deep learning~\cite{ghorbani2017interpretation}, similar to the phenomenon of adversarial examples~\cite{szegedy2013intriguing}. As a direct result, methods built upon Jacobian inherently lack stability guarantees.

Hence, an interesting challenge is to find a principled method to certify and even stabilize Jacobian in a local region. An intuitive method might be an adversarial approach, similar to adversarial examples and learning~\cite{goodfellow14}, that finds the maximum Jacobian distortion (called adversarial Jacobian) around a specified neighborhood, and then try to minimize such distortion. 
Assuming $f$ is twice-differentiable, then Hessian can be utilized for gradient-based methods to find the adversarial Jacobian, which is computationally challenging. Even worse, for the predominantly locally linear neural networks, such as VGG~\cite{simonyan2014very} and residual networks (ResNet)~\cite{he2016deep}, used in computer vision, the Hessian is either ill-defined (on the boundaries of locally linear regions) or $0$ everywhere else.

Fortunately, due to the special functional structure of locally linear neural networks, we discover algorithms that can certify the regions where the Jacobian is stable. Specifically, by exploiting the convexity of a locally linear region, we are able to create a binary search algorithm that find certificate on maximum directional perturbation and $\ell_1$ ball around a point $\bx$ that Jacobian is guaranteed to be stable. In addition, by further exploiting the geometry of locally linear regions, we develop novel analytical algorithm to find the exact certificate on the maximum $\ell_2$ ball around $\bx$ where Jacobian is stable; the algorithm requires computation of the Jacobian of all the neurons with respect to input, which yields a giant computational challenge: naively calling back-propagation for each neuron is intractable. In contrast, we create a novel algorithm that computes the exact Jacobian of all the neurons with respect an input axis by feeding 2 carefully crafted perturbations to the network (in parallel), which does not even require a single call to back-propagation. The computational algorithm can be amortized and parallelized among the input axes that the complexity given $D$ dimensional data is $D+1$ calls to forward pass in parallel.

With the capability to certify the size of locally linear regions, we further develop learning algorithms to expand such locally linear region. Due to the difficulty of the optimization problem, we develop a novel relaxation based on the derivation of primal support vector machine (SVM)~\cite{vapnik1995estimation, cortes1995support}, where the final formulation is resemble to transductive/semi-supervised SVM (TSVM)~\cite{vapnik1977tsvm}. The learning algorithm has the same complexity as the $\ell_2$ certificate problem, which can be computationally challenging in a training scenario when the $D+1$ forward pass cannot be parallelized in one batch (e.g., deep   model on large image). As a result, we develop an unbiased approximate learning algorithm that scales to such high dimensional setting.  

The methods are applicable to a wide range of network architectures as long as the underlying operations consist of affine transformation and piece-wise non-linearities. Empirically, we examine our certificate and learning algorithms with fully-connected (FC), ResNet~\cite{he2016deep}, and recurrent (RNN) networks on image and time-series dataset with qualitative and quantitative experiments.
\ghl{The implementation is in Supplementary Material}
